ALONE: A Dataset for Toxic Behavior among Adolescents on Twitter

The convenience of social media has also enabled its misuse, potentially resulting in toxic behavior. Nearly 66% of internet users have observed online harassment, and 41% claim personal experience, with 18% facing severe forms of online harassment. This toxic communication has a significant impact on the well-being of young individuals, affecting mental health and, in some cases, resulting in suicide. These communications exhibit complex linguistic and contextual characteristics, making recognition of such narratives challenging. In this paper, we provide a multimodal dataset of toxic social media interactions between confirmed high school students, called ALONE (AdoLescents ON twittEr), along with descriptive explanation. Each instance of interaction includes tweets, images, emoji and related metadata. Our observations show that individual tweets do not provide sufficient evidence for toxic behavior, and meaningful use of context in interactions can enable highlighting or exonerating tweets with purported toxicity.

==> Temp/Temp.tex <==
\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal
articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}


%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%

==> dump.tex <==
\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{2.5cm}|p{2.5cm}}
    \toprule[1.5pt]
      \textbf{Kappa} & \textbf{A} & \textbf{B} \\ \midrule
      \textbf{B} & 0.77 & - \\
      \textbf{C} & 0.52 & 0.62 \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Pairwise agreement for the \textbf{three} label scheme, agreement scores between the three annotators (A,B,C) using Cohen Kappa}
\label{tab:cohenannotation1}
\end{table}

\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{2.5cm}|p{2.5cm}}
    \toprule[1.5pt]
      \textbf{Kappa} & \textbf{A} & \textbf{B} \\ \midrule
      \textbf{B} & 0.82 & - \\
      \textbf{C} & 0.49 & 0.63 \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Pairwise agreement for \textbf{two} labels, agreement scores between the three annotators (A,B,C) using Cohen Kappa}
\label{tab:cohenannotation2}
\end{table}

%\FloatBarrier
\begin{table}[!htbp]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
    \toprule[1.5pt]
      \textbf{Number of Tweets} & \textbf{Mean} & \textbf{Minimum} & \textbf{Maximum} \\ \midrule
      Toxic & 13.28 & 3.0 & 304.0 \\ \midrule
      Non-Toxic & 7.15 & 3.0 & 99.0 \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Descriptive statistics of tweets per interaction.}
\label{tab:tweetdatadistribution}
\end{table}

\begin{table}[!htbp]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
    \toprule[1.5pt]
      \textbf{Number of Emoji} & \textbf{Mean} & \textbf{Minimum} & \textbf{Maximum} \\ \midrule
      Toxic & 6.72 & 0.0 & 290.0 \\ \midrule
      Non-Toxic & 3.51 & 0.0 & 60.0 \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Descriptive statistics of emoji per interaction.}
\label{tab:emojidatadistribution}
\end{table}

\begin{table}[!htbp]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
    \toprule[1.5pt]
      \textbf{Number of URLs} & \textbf{Mean} & \textbf{Minimum} & \textbf{Maximum} \\ \midrule
      Toxic & 2.70 & 0.0 & 73.0 \\ \midrule
      Non-Toxic & 1.63 & 0.0 & 26.0 \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Descriptive statistics of URLs per interaction.}
\label{tab:urlsdatadistribution}
\end{table}


\begin{table}[htbp]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
    \toprule[1.5pt]
      \textbf{Number of Images} & \textbf{Mean} & \textbf{Minimum} & \textbf{Maximum} \\ \midrule
      Toxic & 1.18 & 0.0 & 20.0 \\ \midrule
      Non-Toxic & 0.86 & 0.0 & 12.0 \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Descriptive statistics of images per interaction. There were 140 images showing Toxic Behavior and 471 images showing Non-Toxic Behavior.}
\label{tab:imagessdatadistribution}
\end{table}

\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{p{2.5cm}|p{2.5cm}|p{2.5cm}}
    \toprule[1.5pt]
      \textbf{Toxic} & \textbf{Non-Toxic} & \textbf{Unclear} \\ \midrule
      118(17.15\%) & 547(79.51\%) & 23(3.34\%) \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Overall distribution of the data instances over the three labels.}
\label{tab:datadistribution}
\end{table}

\begin{table}[!htbp]
\footnotesize
\begin{center}
\begin{tabular}{p{3cm}p{4cm}}
    \toprule[1.5pt]
      \textbf{Type of URLs} & \textbf{ \# URLs in Toxic Interactions}  \\ \midrule
      Image URLs & 140 (43.88\%) \\ \midrule
      Video URLs & 44 (13.79\%) \\ \midrule
      Text URLs & 48 (15.04\%) \\
     \bottomrule[1.5pt]
\end{tabular}
\end{center}
\caption{Different types of URLs in toxic interactions.}
\label{tab:typesofurlToxic}
\end{table}

%@inproceedings{gaur2019knowledge,
%title={Knowledge-aware assessment of severity of suicide risk for early intervention},
%author={Gaur, Manas and Alambo, Amanuel and Sain, Joy Prakash and Kursuncu, Ugur and Thirunarayan, Krishnaprasad and Kavuluru, Ramakanth and Sheth, Amit and Welton, Randy and Pathak, Jyotishman},
%booktitle={WWW},
%year={2019}
%}

%@article{kursuncu2019modeling,
%  title={Modeling Islamist Extremist Communications on Social Media using Contextual Dimensions: Religion, Ideology, and Hate},
 % author={Kursuncu, Ugur and Gaur, Manas and Castillo, Carlos and Alambo, Amanuel and Thirunarayan, Krishnaprasad and Shalin, Valerie and Achilov, Dilshod and Arpinar, I Budak and Sheth, Amit},
  %journal={ACM-CSCW},
 % year={2019}
%}

%@incollection{kursuncu2019predictive,
 % title={Predictive Analysis on Twitter: Techniques and Applications},
%  author={Kursuncu, Ugur and Gaur, Manas and Lokala, Usha and Thirunarayan, Krishnaprasad and Sheth, Amit and Arpinar, I Budak},
 % booktitle={Emerging Research Challenges and Opportunities in Computational Social Network Analysis and Mining},
 % year={2019}
%}


%@inproceedings{kursuncu2018s,
%  title={What's ur Type? Contextualized Classification of User Types in Marijuana-Related Communications Using Compositional Multiview Embedding},
%  author={Kursuncu, Ugur and Gaur, Manas and Lokala, Usha and Illendula, Anurag and Thirunarayan, Krishnaprasad and Daniulaityte, Raminta and Sheth, Amit and Arpinar, I Budak},
 % booktitle={ACM-IEEE WI},
 % year={2018}
%}

